Option Transfer and SMDP Abstraction with Successor Features

Abstraction plays an important role in the generalisation of knowledge and skills and is key to sample efficient learning. In this work, we study joint temporal and state abstraction in reinforcement learning, where temporally-extended actions in the form of options induce temporal abstractions, while aggregation of similar states with respect to abstract options induces state abstractions. Many existing abstraction schemes ignore the interplay of state and temporal abstraction. Consequently, the considered option policies often cannot be directly transferred to new environments due to changes in the state space and transition dynamics. To address this issue, we propose a novel abstraction scheme building on successor features. This includes an algorithm for transferring abstract options across different environments and a state abstraction mechanism that allows us to perform efficient planning with the transferred options.

==> sections/introduction.tex <==
While reinforcement learning (RL) has recently shown many remarkable successes, e.g., in playing Atari and Go~\cite{mnih2015human,silver2017mastering}, its large sample complexity is still a key problem limiting its applications.
Allowing RL agents to learn transferable and reusable options~\cite{sutton1999between} (i.e., skills) is a promising approach to alleviate the issue of sample complexity. As such, an important problem is to characterise option policies by abstract options that can be transferred and instantiated across different environments. Moreover, planning with abstract options can be particularly useful for many complex, long-horizon planning problems such as the game of Minecraft. 
Figure~\ref{fig:minecraft_baking_scene} illustrates an example scene in Minecraft. In order to obtain a baked potato, the agent can first formulate a simple, abstract plan to collect coal, then collect a potato, and finally perform crafting. Then the agent can instantiate the options by navigating through different rooms to collect the required items. Having acquired the abstract options in a first environment, the agent can also transfer the abstract options and grounds them in an previously unseen environment, then form an abstract semi-Markov Decision Process (SMDP) for planning using the transferred options, cf.~Figure~\ref{fig:abstract_mdp_graphs_smaller} for an example.


In this work, we propose abstract option representations that can be: (1) shared across different environments, (2) grounded in unseen environments with a certain precision, and (3) used for planning with near-optimal performance.

% CHALLENGES + THE GAP
In the context of RL, options are described by policies which are typically not transferable due to new state spaces and transition dynamics. This issue is underlined by the fact that abstract options such as \emph{``open a door''} can often correspond to different policies in different MDPs. To enable transferable abstract options, we define shared \emph{features} across different environments (e.g., doors), and abstract options as successor features (SF)~\cite{dayan1993improving,barreto2016successor}, which captures the feature expectations of the option trajectories. 
One way of grounding such an abstract option could be through finding an option policy which maximises a preference function over the successor features~\cite{barreto2019option}. However, such rewards may yield imprecise option behaviours due to the interference between the different components of the feature, hence the preference function needs to be carefully hand-crafted in unseen environments in order to produce an intended option behaviour (e.g., to acquire all required feature components before terminating).
To address these issues, we formulate option grounding as a feature-matching problem where the feature expectations of the learned option match the abstract option. More specifically, we adapt techniques from inverse reinforcement learning (IRL), and present an algorithm which finds ground options efficiently with a specified precision. 
Finally, we demonstrate that the abstract options can be used for SMDP planning with near-optimal performance. 

% Structure:
This paper is structured as follows: in Section~\ref{sec:background} we introduce the background, we define the abstract option representations in Section~\ref{subsec:abstract_options} and the grounding algorithms
in Section~\ref{subsec:lifting_options}.
In Section~\ref{sec:abstraction}, we introduce our SMDP abstraction framework which produces an abstract SMDP model for planning. Our empirical results are presented in Section~\ref{sec:experiments}, a discussion with related work in Section~\ref{sec:related workd}, and we conclude our paper in Section~\ref{sec:conclusion}. %The code for the algorithm will be released upon publication.


%\begin{figure}
%    \centering
%    \includegraphics[width=0.5\textwidth]{img/illustration.pdf}
%    \caption{Motivating Example}
%    \label{fig:illustration}
%\end{figure}

==> sections/proof_backup.tex <==
\subsection{Proofs}
The multi-step transition probability is defined similarly to the single-step transition probability.
The transition probability from $s_i$ to (terminating in) $s_j$ through option $o$ is defined as the successor representation of option $o$ starting from $s_i$ towards state-actions $(s_j, a_\textnormal{term})$:
\begin{align}
    P^T(s_i, s_j, o) = \sum_{k=1}^{\infty}\gamma^k P^T(s_i, s_j, o, k) = \psi^o(s_i, s_j, a_T)
\end{align}
where $P(s_i, s_j, o, k)$ is the probability of option o starting in $s_i$ and terminating in $s_j$ after $k$-steps.

Therefore, the Q-value of an option is defined as:
\begin{align}
    Q(s_i, o) 
        &= \mathbb{E}[r_{s_i, o} + \gamma^k \max_{o_j}Q(s_j, o_j)]\\
        &= r_{s_i, o} + \sum_{s_j\in S}\sum_{k=1}^{\infty} \gamma^k P^T(s_i, s_j, o, k) \max_{o_j}Q(s_j, o_j)\\
        &= r_{s_i, o} + \sum_{s_j\in S}P^T(s_i, s_j, o) \max_{o_j}Q(s_j, o_j)
\end{align}
Therefore, a multi-step homomorphism which is similar to single-step MDP homomorphism:
\begin{align}
    \forall \phi(s_1) = \phi(s_2), g(o_1) = g(o_2),  S'_A, \qquad
    \sum_{s_j\in S'_A} P^T(s_1, s_j, o_1) &= \sum_{s_j\in S'_A} P^T(s_2, s_j, o_2), and \phantom{----------} \label{eq: homomorphism_prob}\\
    r_{s_1, o_1} &= r_{s_2, o_2} \label{eq: homomorphism_reward}
\end{align}
While a multi-step $Q^*$ abstraction is more like 
\begin{align}
    \forall f(s_1) = f(s_2), g(o_1) = g(o_2),  \qquad
    Q(s_1, o_1) = Q(s_2, o_2)\\
\end{align}

\subsection{Successor homomorphism through Options (w. termination)}
To define the homomorphism which achieves Eq.\eqref{eq: homomorphism_prob}\eqref{eq: homomorphism_reward}, we can use the successor representation of options.
\dongge{How we define the successor homomorphism would be important, though type 1 and 2 can both lead to the multi-step homomorphism, and type 3 using successor features can be related to type 2 or type 1.}
\subsubsection{Type 1: Successor representation as termination probability + feature-matching options}
This means that the probability of the option terminating in another abstract state is the same across all ground states in an abstract state. The reward equality part comes from the options having equal feature.
\begin{align}
    &\phi(s_1) = \phi(s_2) \implies \forall S'_A, g(o_1) = g(o_2) = o_A  \\ 
    &(i) \sum_{s_j\in S'_A} P(s_1, s_j, o_1) = \sum_{s_j\in S'_A}P(s_2, s_j, o_2), \textnormal{ where } P(s_1, s_j, o_1) = \sum_{k=1}^{\infty} \gamma^k P(s_1, s_j, o_1, a_k = a_T) = \mu_{s_j, a_T} \\
    &(ii) \textnormal{ Feature matching: }\theta_{o_1} = \theta_{o_2} \implies r_{s_1, o_1} = r_{s_2, o_2} 
\end{align}
\iffalse
\subsubsection{Type 2: Abstract termination state distribution}
This extends the 'terminating' action to all actions. The reward equality part comes from the options having equal feature.
\begin{align}
    &\phi(s_1) = \phi(s_2) \implies \forall S'_A, a_j, g(o_1) = g(o_2) = o_A  \\ 
    &(i) \sum_{s_j\in S'_A} P(s_1, s_j, a_j, o_1) = \sum_{s_j\in S'_A}P(s_2, s_j, a_j, o_2) \textnormal{ where } P(s_1, s_j, a_j, o_1) = \sum_{k=1}^{\infty} \gamma^k P(s_1, s_j, o_1, a_k = a_j) = \mu_{s_j, a_j}\\
    &\implies r_{s_1, o_1} = r_{s_2, o_2} \textnormal{ and } \sum_{s_j\in S'_A} P(s_1, s_j, a_T, o_1) = \sum_{s_j\in S'_A}P(s_2, s_j, a_T, o_2)
\end{align}\fi

\subsubsection{Type 2: Ground termination states distribution}
This would be most like the successor similarity, where the successor representation generated by an option from any ground state in an abstract state are equal. Both reward and transition probability equality come from the homomorphism, so no requirement on the option mapping $g(o)$.
\begin{align}
    &\phi(s_1) = \phi(s_2) \implies \forall S'_A, a_j, g(o_1) = g(o_2) = o_A  \\ 
    &(i) P(s_1, s_j, a_j, o_1) = P(s_2, s_j, a_j, o_2)\\
    &(ii) \sf_{s_1, o_1} = \sf_{s_2, o_2} 
\end{align}

\subsubsection{Type 3: Partial homomorphism through Successor Feature Options (relaxation from Type 2)}
Like in the SMDP homomorphism paper, many times, a complete homomorphism of the environment does not exist. However, there can be many partially homomorphic regions, where a similar high-level option can be initiated. By matching each option segment, we can also estimate the total deviation from the whole option. We relax the equality of successor representation generated by an option to the equality of successor feature generated.
\begin{align}
    \phi(s_1) = \phi(s_2) \implies \forall  g(o_1) = g(o_2) = o_A, \qquad
    \theta(s_1, o_1) = \theta(s_2, o_2),
\end{align}
where $o_1$ and $o_2$ can be executed in states $s_1$ and $s_2$, respectively.
There is no guarantee on the abstract transition probability, but the reward equality still holds. The implicit assumption (relaxing from Type 2 successor representation) is that an option achieving the same successor feature will generate a similar successor representation (state-action visitation frequency). And hence, the option will achieve the same immediate reward, and lead to similar abstract next states. The advantage over SR similarity is the transferability, and also avoiding matching SR on each $(s, a)$ pair (instead, we match to the $(s,a)$ pair features, so automatically grouping together equivalent $(s,a)$ pairs.)

\subsubsection{Type 4: successor representation/features for all possible policies (instead of options)} 
This is outside the context of options, where we do not consider the termination of an option, so no need for the termination probability to be matched.
\begin{align}
    &\phi(s_1) = \phi(s_2) \implies \forall g(\pi_1) = g(\pi_2) = \pi_A  \\ 
    &(i) P(s_1, s_j, a_j, \pi_1) = P(s_2, s_j, a_j, \pi_2) \textnormal{ where } P(s_1, s_j, a_j, \pi_1) = \sum_{k=1}^{\infty} \gamma^k P(s_1, s_j, \pi_1, a_k = a_j) = \mu_{s_j, a_j}\\
    &\implies V(s_1, \pi_1) = V(s_2, \pi_2)
\end{align}

\subsection{Error bounds similar to MDP homomorphism}
Whichever successor homomorphism type we assume, once we reach the multi-step homomorphism as Eq.\eqref{eq: homomorphism_prob},\eqref{eq: homomorphism_reward}, we can do the error bounds similar to the single-step cases like \cite{abel2016near} or \cite{li2006towards}:

\noindent
\textbf{Exact equality} \cite{li2006towards} Theorem 3: With abstractions $\phi_{model}$, $\phi_{Q^\pi}$, $\phi_{Q^*}$, the optimal abstract policy is optimal.

\noindent
\textbf{$\epsilon$-equality:} In \cite{abel2016near}, an error bound for $\phi_{model}$ can be derived by transforming it to $\phi_{Q^*}$.

We can derive the error bounds similarly given a multi-step $\epsilon$-homomorphism:

\subsubsection{Step 1: Show that $|Q_A(s_A, o_A) - Q_G(s_1, o_1)|\leq \frac{\epsilon}{1-\gamma}.$}
\begin{align}
    \textbf{Given: } &\textnormal{Abstraction: } P^T(s_A, s'_A, o'_A) = \sum_{s_i\in s_A} w_{s_i}\sum_{s_j\in s'_A} P^T(s_i, s_j, o_i), \textnormal{ and } r_{s_A, o'_A}= \sum_{s_i\in s_A} w_{s_i} r_{s_i, o_i}
    \\ &\textnormal{Homomorphism: } \phi(s_1) = \phi(s_2) = s_A, g(o_1) = g(o_2) = o_A \implies\\
    &\textnormal{(i) } |\sum_{s_j\in s'_A} P^T(s_1, s_j, o_1) - \sum_{s_j\in s'_A}P^T(s_2, s_j, o_2) | \leq \epsilon_\psi\\
    &\textnormal{(ii) } |r(s_1, o_1) - r(s_2, o_2)| \leq \epsilon_\theta
\end{align}
\begin{proof}
\begin{align}
    &Q_A(s_A, o_A)
        = \mathbb{E}_{o_A}[r_{s_A, o_A} + \gamma^k \max_{o'_A}Q(s'_A, o'_A)] 
        = \sum_{s_i\in s_A}w_{s_i} r_{s_i, o_i} + \sum_{s_i\in s_A} w_{s_i} \sum_{s'_A}\sum_{s_j\in s'_A} P^T(s_i, s_j, o) \max_{o'_A}Q(s'_A, o'_A)\\
    &Q_G(s_1, o_1)
        = \mathbb{E}_{o_1}[r_{s_1, o_1} + \gamma^k \max_{o'_j}Q(s'_j, o'_j)]
        = r_{s_1, o_1} + \sum_{s'_A}\sum_{s_j\in s'_A} P^T(s_1, s_j, o) \max_{o'_A}Q(s_j, o'_j)
\end{align}
\begin{align}
    &|Q_A(s_A, o_A) - Q_G(s_1, o_1)|\\
        &= \sum_{s_i\in s_A}w_{s_i} (r_{s_i, o_i} - r_{s_1, o_1}) + 
        \sum_{s_i\in s_A} w_{s_i} \sum_{s'_A}\sum_{s_j\in s'_A} \left( P^T(s_i, s_j, o_A) \max_{o'_A}Q(s'_A, o'_A) - P^T(s_1, s_j, o_1) \max_{o'_j} Q(s'_j, o'_j)\right)\\
        &\leq \underbrace{\epsilon_\theta + \sum_{s_i\in s_A} w_{s_i} \sum_{s'_A}\sum_{s_j\in s'_A} \left( P^T(s_i, s_j, o_A) \max_{o'_A}Q(s'_A, o'_A) - P^T(s_1, s_j, o_1) \max_{o'_A} Q(s'_A, o'_A)\right)}_{(1)}\\ 
        &+ \underbrace{\sum_{s_i\in s_A} w_{s_i} \sum_{s'_A}\sum_{s_j\in s'_A} P^T(s_1, s_j, o_1) \left(\max_{o'_A} Q(s'_A, o'_A)- \max_{o'_j} Q(s'_j, o'_j)\right)}_{(2)}
\end{align}
\begin{align}
    (1)
        &= \epsilon_\theta + \sum_{s_i\in s_A} w_{s_i} \sum_{s'_A}\sum_{s_j\in s'_A} \left( P^T(s_i, s_j, o) - P^T(s_1, s_j, o_1)\right) \max_{o'_A} Q(s'_A, o'_A) \phantom{---------------}\\
            &\leq \epsilon_\theta + \sum_{s'_A}\epsilon_\psi \max_{o'_A} Q(s'_A, o'_A)
        \leq \epsilon_\theta+\frac{|S_A|\epsilon_\psi}{1-\gamma}\\ &\textnormal{ Denote as } \epsilon = \epsilon_\theta+\frac{|S_A|\epsilon_\psi}{1-\gamma} \textnormal{ , note that if options are typically long, then $\epsilon_\psi \approx \gamma^k$ where $k$ is the number of steps.}\\
        &\textnormal{Alternatively, if no guarantees on the transition probability is provided, } \sum_{s'_A}\sum_{s_j\in s'_A} P^T(s_i, s_j, o) \leq \gamma (\approx \gamma^k)\\
        &\textnormal{ we can approximate (1) by } \approx\epsilon_{\theta} + \frac{\gamma^k}{1-\gamma^k}. \\
    (2)
        &= \underbrace{\sum_{s'_A}\sum_{s_j\in s'_A} P^T(s_1, s_j, o_1)}_{(3)\leq\gamma, (\approx \gamma^k)}\left( \max_{o'_A}Q(s'_A, o'_A) - \max_{o'_j}Q(s'_j, o'_j)\right)\\
        &\leq \gamma \max_{s'_A}[|Q(s'_A, o^*_A) - Q(s'_j, o^*_j)|]
\end{align}
(3) is since the option terminates with probability 1:  $\sum_{s'_A}\sum_{s_j\in s'_A} \sum_{k=1}^{\infty} P^T(s_1, s_j, o_1, k) = 1$

And $\sum_{s'_A}\sum_{s_j\in s'_A} P^T(s_1, s_j, o_1) = \sum_{s'_A}\sum_{s_j\in s'_A} \sum_{k=1}^{\infty} \gamma^k P^T(s_1, s_j, o_1, k)$

Therefore, $\sum_{s'_A}\sum_{s_j\in s'_A} P^T(s_1, s_j, o_1) \leq \gamma.$ 

Moreover, if an option typically lasts for $k$ steps, then  $\sum_{s'_A}\sum_{s_j\in s'_A} P^T(s_1, s_j, o_1) \approx \gamma^k$.

\begin{align}
    |Q_A(s_A, o_A) - Q_G(s_1, o_1)| 
        &\leq (1) + (2) 
        \leq  \epsilon + \gamma \max_{s'_A}[|Q(s'_A, o^*_A) - Q(s'_j, o^*_j)|] \\
        &\leq \epsilon + \gamma[\epsilon + \gamma\max_{s'_A}[|Q(s'_A, o^*_A) - Q(s'_j, o^*_j)|]\\
        & \leq \ldots \approx \frac{\epsilon}{1-\gamma}
\end{align}
Also if we assume options typically take $k$ steps, then we can approximate the error bound and substitute $\gamma$ with $\gamma^k$.
\end{proof}

\subsubsection{Step 2: The optimal option in the abstract MDP has a Q-value in the ground MDP that is nearly optimal:}

From step 1, we have $|Q_A(s_A, o_A) - Q_G(s_1, o_1)| \leq \frac{\epsilon}{1-\gamma}$.
\begin{align}
    &\textnormal{By definition of optimality, } Q_A(s_A, g(o^*_1)) \leq Q_A(s_A, o^*_A) \implies Q_A(s_A, g(o^*_1)) + \frac{\epsilon}{1-\gamma} \leq Q_A(s_A, o^*_A) + \frac{\epsilon}{1-\gamma}\\
    & \textnormal{Therefore, by step 1 then by optimality: } Q_G(s_1, o^*_1) \leq Q_A(s_A, g(o^*_1)) + \frac{\epsilon}{1-\gamma} \leq Q_A(s_A, o^*_A) + \frac{\epsilon}{1-\gamma}\\
    & \textnormal{Again by step 1: } Q_A(s_A, o^*_A)  \leq Q_G(s_1, g^{-1}(o^*_A)) + \frac{\epsilon}{1-\gamma}\\
    &\textnormal{Therefore, } Q_G(s_1, o^*_1) \leq Q_A(s_A, o^*_A) + \frac{\epsilon}{1-\gamma} 
    \leq Q_G(s_1, g^{-1}(o^*_A)) + \frac{2\epsilon}{1-\gamma}
\end{align}
This shows that the optimal option $o^*_A$ in the abstract MDP is also nearly optimal in the ground MDP.

\subsubsection{Step 3: The optimal SMDP policy in the abstract MDP yields near optimal performance in the ground MDP:}
Let the ground policy lifted from the abstract policy of the options be defined as $g^{-1}(\pi^*_A)$
\begin{align}
    &Q^{\pi^*_G}(s, o^*) - Q^{g^{-1}(\pi^*_A)} (s, g^{-1}(o^*_A))\\
        &\leq \frac{2\epsilon}{1-\gamma} + Q^{\pi^*_G}(s, g^{-1}(o^*_A)) - Q^{g^{-1}(\pi^*_A)} (s, g^{-1}(o^*_A)) \textnormal{ , by step 2}\\
        &= \frac{2\epsilon}{1-\gamma} + [r_{s, g^{-1}(o^*_A)} + \sum_{s'\in S} P^T(s, s', g^{-1}(o^*_A)) Q^{\pi^*_G}(s', o^*_{s'})] - [r_{s, g^{-1}(o^*_A)} + \sum_{s'\in S} P^T(s, s', g^{-1}(o^*_A)) Q^{g^{-1}(\pi^*_A)}(s', g^{-1}(o^*_{s_A'}))]\\
        &= \frac{2\epsilon}{1-\gamma} +  \sum_{s'\in S} P^T(s, s', g^{-1}(o^*_A)) [Q^{\pi^*_G}(s', o^*_{s'}) -  Q^{g^{-1}(\pi^*_A)}(s', g^{-1}(o^*_{s_A'}))]\\
        &\leq \frac{2\epsilon}{1-\gamma} + \gamma \max_{s'\in S}[|Q^{\pi^*_G}(s', o^*_{s'}) - Q^{g^{-1}(\pi^*_A)}(s', g^{-1}(o^*_{s'_A}))|]\\
        &\leq \frac{2\epsilon}{1-\gamma} + \gamma\max_{s'\in S}[\frac{2\epsilon}{1-\gamma} + Q^{\pi^*_G}(s', g^{-1}(o^*_{s'_A})) - Q^{g^{-1}(\pi^*_A)} (s', g^{-1}(o^*_{s'_A}))] \textnormal{ , by step 2}\\
        &\leq \frac{2\epsilon}{1-\gamma} + \gamma \frac{2\epsilon}{1-\gamma} + \gamma^2 \frac{2\epsilon}{1-\gamma} \ldots\\
        &\leq \frac{2\epsilon}{(1-\gamma)^2}
\end{align}
As discussed above, if an option typically takes $k$ steps, then the error bound would be approximately $\frac{2\epsilon}{(1-\gamma^k)^2}$. The main error source is in multi-step immediate (option) reward from the option feature matching.


==> sections/table.tex <==
\begin{table*}[t]
\centering
\begin{minipage}[b]{0.48\linewidth}
\input{sections/algorithm_original}
\end{minipage}
\hfill
\begin{minipage}[b]{0.48\linewidth}
\resizebox{1.\linewidth}{!}{%

\renewcommand{\arraystretch}{1.} %%% Default value: 1
\begin{tabular}{@{}cccccccc@{}}
\toprule
 &  & \multicolumn{2}{c}{2 Rooms} & \multicolumn{2}{c}{3 Rooms} & \multicolumn{2}{c}{4 Rooms} \\ \cmidrule(l){3-8} 
 &  & $\Delta\sf^o$ & \textit{LP} & $\Delta\sf^o$ & \textit{LP} & $\Delta\sf^o$ & \textit{LP} \\ \midrule
\multirow{3}{*}{Find Key} & \textit{IRL-naive} & 0.0 & 157 & 0.0 & 487 & 0.0 & 1463 \\
 & \textit{IRL-batch} & \textbf{0.0} & \textbf{2} & \textbf{0.0} & \textbf{2} & \textbf{0.0} & \textbf{2} \\
 & \textit{ok}~\cite{barreto2019option} & 0.002 & - & 0.06 & - & 0.04 & - \\ \midrule
\multirow{3}{*}{Find Star} & \textit{IRL-naive} & 0.0 & 157 & 0.0 & 487 & 0.0 & 1463 \\
 & \textit{IRL-batch} & \textbf{0.0} & \textbf{2} & \textbf{0.0} & \textbf{2} & \textbf{0.0} & \textbf{2} \\
 & \textit{ok}~\cite{barreto2019option} & 0.007 & - & 0.04 & - & 0.06 & - \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Find Key, \\ Open Door\end{tabular}} & \textit{IRL-naive} & 0.0 & 157 & 0.0 & 487 & \textbf{0.0} & 1463 \\
 & \textit{IRL-batch} & \textbf{0.0} & \textbf{3} & \textbf{0.0} & \textbf{15} & 0.041 & \textbf{29} \\
 & \textit{ok}~\cite{barreto2019option} & 0.34 & - & 0.433 & - & 0.211 & - \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Find Key, \\ Open Door, \\ Find Star\end{tabular}} & \textit{IRL-naive} & 0.0 & 157 & 0.0 & 487 & 0.08 & 1463 \\
 & \textit{IRL-batch} & \textbf{0.0} & \textbf{4} & \textbf{0.0} & \textbf{16} & \textbf{0.004} & \textbf{7} \\
 & \textit{ok}~\cite{barreto2019option} & 0.902 & - & 1.028 & - & 0.691 & - \\ \bottomrule
\end{tabular}
}
\caption{Performance and efficiency of option grounding in the Object Rooms domain. 
%\sebastian{Explain quantities. Is the value of $\epsilon$ important? }} 
%Abstract options encoded from demonstration in a 2-room environment are transferred to target environments with 2 - 4 rooms. 
%\emph{enum.} is the ground truth approach (Algo.~\ref{algo:lifting_original}), by enumerating all starting states, while \emph{IRL-batch} is the IRL-batched approach (Algo.~\ref{algo:lifting_IRL-batch}).
$\Delta\sf^o$ is the average feature difference between the computed options and an optimal ground truth option policy over all starting states in the initiation set. } %The results show that the IRL-IRL-batch can find the optimal options as the ground truth (IRL-naive) while significantly reducing the number of LP solved.}
\label{table:key_door_option_fitting}
\end{minipage}%
\vspace{-3mm}
\end{table*}
